Object-Aware Cropping for Self-Supervised Learning

A core component of the recent success of self-supervised learning is cropping data augmentation, which selects sub-regions of an image to be used as positive views in the self-supervised loss. The underlying assumption is that randomly cropped and resized regions of a given image share information about the objects of interest, which the learned representation will capture. This assumption is mostly satisfied in datasets such as ImageNet where there is a large, centered object, which is highly likely to be present in random crops of the full image. However, in other datasets such as OpenImages or COCO, which are more representative of real world uncurated data, there are typically multiple small objects in an image. In this work, we show that self-supervised learning based on the usual random cropping performs poorly on such datasets. We propose replacing one or both of the random crops with crops obtained from an object proposal algorithm. This encourages the model to learn both object and scene level semantic representations. Using this approach, which we call object-aware cropping, results in significant improvements over scene cropping on classification and object detection benchmarks. For example, on OpenImages, our approach achieves an improvement of 8.8% mAP over random scene-level cropping using MoCo-v2 based pre-training. We also show significant improvements on COCO and PASCAL-VOC object detection and segmentation tasks over the state-of-the-art self-supervised learning approaches. Our approach is efficient, simple and general, and can be used in most existing contrastive and non-contrastive self-supervised learning frameworks.

==> LaTeX/Images/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> LaTeX/Images/methods.tex <==
\section{Proposed Approach}
\label{sec:model}
%Our hypothesis is that scene cropping has a high likelihood of including a lot of information irrelevant to the object. This effect is more pronounced when the objects are small relative to the size of the image. 
% of missing objects when the objects are small relative to the size of the image. 
%This leads to suboptimal representations for OpenImages due to the inclusion of data that is weakly correlated with the objects of interest. 

Our analysis shows that SSL methods based on either purely object crops, or purely scene crops, both perform worse than supervised learning. This suggests a third option: incorporating \emph{both} object and scene information in the crops. Our hypothesis is that context around an object is helpful to learn robust representations due to the natural correlations between scene and object \citep{Hinton2021HowTR}. However, it is unclear what mix of object and scene information is most helpful in learning robust representations. Our main contribution is a simple and effective approach to achieving this cropping mechanism. We also experiment with a number of plausible baselines to incorporate scene and object information.

To enable object-awareness, we consider three object proposal models: BING \citep{Cheng2014BINGBN} and Edge-Boxes \citep{Zitnick2014EdgeBL}, both of which are trained with boxes from Pascal-VOC; and an unsupervised object proposal method \citep{vo2019unsupervised}. BING \citep{Cheng2014BINGBN} uses the norm of gradients within a fixed window size as a simple feature that is fed into a cascaded SVM framework to make object proposals. This method is trained on the ground-truth bounding boxes of $2501$ images of the PASCAL-VOC \citep{everingham2010pascal} training set. Note that BING does not use any class label, but only label independent bounding box information. BING has the advantage of extremely fast performance (>$125$ fps on an image of size $300 \times 300$), generates many proposals, and generalizes well to many datasets, as shown in \citet{Cheng2014BINGBN} and seen in our empirical results. This makes BING well suited as an object proposal algorithm. In our experiments, we generate up to $10$ proposals per image and select one object uniformly at random among these proposals. The details of other object proposals are present in supplementary Section \ref{sec:object_proposal_methods}. Our results in Table \ref{tab:voc_moco} show that other object proposal methods provide sufficient quality and the choice may be mostly dependent on the speed of the method. We experiment with four types of cropping in the rest of the paper: 

%Due to the fast performance of BING, we use it in all subsequent experiments. 

%Objects with well-defined closed boundaries are strongly correlated large gradient norms. Objectness of an image window, they resize it to 8 × 8 and use the norm of the gradients as a simple 64D feature  for learning a generic objectness measure in a cascaded SVM framework. They further use a binarized version of the Normed Gradient features to significantly speed up their processing. BING relies on the low-level cues concerning the object boundaries and has been shown to be very generalizable and can predict category independent object proposals. BING has been shown to effective in plethora of tasks such as multi-label image classification \citep{Wei2016HCPAF}, semantic segmentation \citep{pinheiro2015imagelevel}, video-classification \citep{zha2015exploiting}, co-salient object detection \citep{ZhangSaliency}, deep multi instance learning \citep{7298968} and video-summarization \citep{Lee_2015}. The high efficiency and speed of BING makes it suitable for  generating object proposals in our datasets. So, we use BING and generate 10 proposals for every image in the OpenImages-Subset and MS-COCO \citep{Lin2014MicrosoftCC} datasets. We randomly pick one out of the 10 generated proposals as a positive sample and Random-Resized crop as other positive sample. We then train MOCOV2 \citep{chen2020improved} and BYOL \citep{grill2020bootstrap} on both of these datasets.
% We used these bounding boxes to pre-train MOCO so that we are able to work on non-iconic datasets like OpenImages \cite{Kuznetsova_2020}. \\


%Unsupervised object discovery methods try to detect the objects present in an image and also structure of the object collection \citep{vo2019unsupervised,cho2015unsupervised} in a completely unsupervised manner. Similar to BING we use \citep{vo2019unsupervised} to generate object proposals. \citep{vo2019unsupervised} uses a robust matching technique which relies on appearance and geometric consistency constraints to assign confidence and saliencey scores to region proposals. However as compared to BING this method is very slow and unlike BING is very difficult to plug in into various deep learning pipelines. Hence we mostly focus on using BING as our default proposal generation method.


%\subsection{Proposed method}
% % \TODO{add object random crop baseline information which used GT boxes}
% We now discuss the different type of cropping which we consider for an image.

% For training contrastive SSL methods, we treat the randomly cropped patches on the pairs of images selected these cropping strategies as positive views of a given image and other randomly sampled images as negative views. 
% Note that for creating positive samples we randomly crop on output from both the cropping strategies.
% in the mini-batch
% We begin by describing methods which take in extra context and scene level information followed by other object level methods. 

%To achieve this we treat the proposals given by BING as object crops and random-resized crops as scene crops.
%Our aim is to learn both object and scene level representations, to this end we consider three kinds of combinations of cropping; Object-Scene cropping, Object-Object cropping and Scene-Scene cropping. Now we discuss these methods in detail:\\

% \textbf{Adding context and scene level information:}
% To add scene level information we try two different methods. We now describe both of these methods in detail. 

\textbf{(a) Dilated object proposals (Obj-Obj+Dilate Crop):} 
Scene pixels spatially close to the object are more likely to have a positive correlation with the object. With this intuition, we generate the second view by dilating the BING proposal. We dilate the box by $10\%$ or $20\%$ of the image size, followed by a random crop. Changing $\delta$ gives us control over how much scene information is incorporated (a value of $10\%$ works well in most cases). Note that the original and dilated boxes are both followed by a random crop, ensuring that the first view is not trivially included in the second view. The choice of which crop to use as query or key is arbitrary and both object and dilated object crops can be used as either key and query.  We also consider other baselines listed below which are other plausible approaches to incorporating scene information. However, as shown in the results Section \ref{secc:results}, dilated crops are the best performing method. 

\textbf{(b) Scene-Scene Crop}: We take two random crops in an image and treat them as positive views. This is the default approach used in MoCo-v2 and other SSL approaches. From our analysis in Section \ref{sec:analysis}, this approach performs poorly on datasets such as OpenImages. 

\textbf{(c) Shifted object proposals (Obj-Obj+Shift Crop)}: Unlike Obj-Obj+Dilate, here, the second view is a box selected at random within a pre-specified distance range of the first box (the BING proposal). To choose a pre-specified distance, we choose a random value for the offset from a few ranges: $80$-$100$ pixels; $100$-$120$ pixels etc. 

% Object-Object crop in principle is similar to standard cropping used in SSL approaches like MoCo-v2 \citep{chen2020improved} on ImageNet, since the crops have good amount of overlap with the object.   
% One potential drawback of an object-focused crop is that it ignores context information (scene) which can be useful in disambiguating objects that may be occluded or blurry. 

% \textbf{Value of lower scale of Random-Resized crop for object crops:}
% The Object-Crop usually are not very small and cover a decent portion of the image; on COCO dataset it covers about 39\% of the image and on OpenImages it cover 23\% of the image. So, we instead of using standard scale of 0.2 as the lower scale, we calculate the scale for every dataset. For ex. in case of COCO dataset, since object crops cover 40\% of the image we use 0.4 as the lower scale. Similarly, in case of OpenImages we use 0.2 as the lower scale since object crops cover close to 20\% of the image.
\textbf{(d) Random crop (Obj-Scene Crop):} The first view is the BING proposal; and a regular random crop at scene level is the second view. This method provides information at both object and scene levels, and we use it as a baseline for adding context information to the model. 
%Our hypothesis is that this approach to cropping should result in better representations since it encompasses object-centric and contextual (scene) information. Our experiments in Section \ref{secc:results} support this hypothesis. 

% Let's denote the dilation by $\delta$, and the height and width of the image by $H,W$.  The vertices of the BING crop in the original image are $X_1,Y_1$(top left corner) and $X_2,Y_2$(bottom right corner). So the size of dilated crops will be. 
% \begin{eqnarray*}
% X_1\_dilated = X_1\_dilated - \delta * W , 
% Y_1\_dilated = Y_1\_dilated - \delta * H \\
% X_2\_dilated = X_2\_dilated + \delta * W ,
% Y_2\_dilated = Y_2\_dilated + \delta * H
% \end{eqnarray*}
\paragraph{Discussion on lower scale of random resized crop:}
As stated above, for both the Obj-Obj+Dilate and Obj-Obj+Shift crops, we use a random crop on the BING object proposal or its shifted or dilated version, to generate the final views. Since the object proposal itself is a small fraction of the image (e.g. in COCO, an object crop typically covers about 39\% of the image), using the usual default lower value for the random crop range (usually $0.2$) works poorly as it results in extremely small crops from the image. Therefore, we set the lower limit such that it matches the minimum sized crop in case of the usual scene crop ($s_{\text{min}} = \frac{0.2}{\text{average BING proposal size}}$) . 

%For ex. in case of COCO dataset, since object crops cover 40\% of the image we use 0.4 as the lower scale. Similarly, in case of OpenImages we use 0.2 as the lower scale since object crops cover close to 20\% of the image.

% \textbf{OARC-Scene Crop using dilation}: \\


% \textbf{Combining all three crops}: We also experiment with combining the $3$ approaches above by randomly sampling any one of these crop types with equal probability. This approach leads to very minimilastic overhead and gives good performance on COCO and OpenImages datasets. 
% In practice we find that it does performs similar to and in some cases slightly better than the simpler object-scene crop approach above.

%\textbf{Different projection heads for Object and Scene crops:}
\paragraph{Different projection heads for Object and Scene crops:}
The projection head, introduced in \citet{chen2020simple} is an important component of most SSL methods. This is a deep network that maps representations from the encoder backbone to a lower-dimensional space where the loss function is applied. In \citet{chen2020exploring}, a single projection head is used for both views. We find it beneficial for performance to use two different projection heads: one for the first view (BING crop) and another for the second view for obj-scene, obj-obj+dilate and obj-obj+shift crops. For scene-scene crops we always use a single projection head. We hypothesize that the different projection networks specialize to either an object-specific representation, or to a representation that incorporates scene information. 

%$\bm z_i = g(\bm h_i)=W^{(2)}\sigma(W^{(1)}\bm h_i)$ where $\sigma$ is a ReLU non-linearity, and $\bm h_i = f(\tilde{\bm x}_i) = \mathrm{ResNet}(\tilde{\bm x}_i)$ where $\bm h_i\in \mathbb{R}^d$ is the output after the average pooling layer. They show that $g(\cdot)$ can remove information that may be useful for the downstream task, such as the color or orientation of objects.  We hypothesize that Object and Scene crops often contain different object orientation and color information; hence we propose to use different projection heads for scene and objects. This gives us
% \begin{eqnarray*}
%$\bm z\_obj = (W_{object}^{(2)}\sigma(W_{object}^{(1)}\bm h_i))$
%and $\bm z\_scene = (W_{scene}^{(2)}\sigma(W_{scene}^{(1)}\bm h_i))^T $.
% \end{eqnarray*}

Other than the above change to the cropping methodology, we leave the rest of the SSL pipeline unchanged: other data augmentations such as color shifts are applied in the usual manner, and the loss functions and training regimes are also unchanged. Our approach therefore involves really simple changes to most SSL pipelines, involving only a few lines of code. 





==> LaTeX/Images/openimages.tex <==
\section{Analysis of Self-Supervised Learning methods on the OpenImages Dataset}

\label{sec:analysis}
In this section, we first identify some limitations of state-of-the-art SSL methods such as MoCo-v2  \citep{he2019momentum,chen2020improved}, SwAV  \citep{NEURIPS2020_70feb62b} and BYOL \citep{grill2020bootstrap} on non-iconic datasets. These methods have nearly closed the performance gap with supervised learning methods when pre-trained and linear probed on ImageNet \citep{imagenet_cvpr09}. However, the performance of these methods on non-iconic datasets (where images contain multiple small objects) has not been extensively studied. OpenImages \citep{kuznetsova2020open} is such a dataset, with images of complex scenes and several objects (containing, on average, $8$ annotated objects per image). It consists of a total of $9.1$ million images. To perform controlled experiments on the effectiveness of cropping on SSL method performance, we construct a subset of the OpenImages dataset. We sample images that have labelled bounding boxes to enable comparisons with fully supervised learning. Secondly, we sample images with objects from at least $2$ distinct classes to create a dataset that better reflects real-world uncurated data. Finally,  we only consider class categories with at least 900 images to mitigate effects of imbalanced class distribution. After this processing, we have $212,753$ images present across $208$ classes and approximately $12$ objects per image on average. We provide further details in the supplementary Sec \ref{sec:details_openimages}. For convenience, we still refer to this dataset as OpenImages through this paper. %We begin by showing the results of the state-of-the-art methods on OpenImages-Subset.


\subsection{Performance of SSL methods}
\label{sec:sslanalysis}
% We pretrain several state-of-the-art SSL methods MoCo-v2 \citep{he2019momentum,chen2020improved}, CMC \citep{tian2019contrastive}, SwAV  \citep{NEURIPS2020_70feb62b} and BYOL \citep{grill2020bootstrap} on our OpenImages dataset. MoCo \citep{he2019momentum} is a contrastive learning-based SSL approach that uses data augmentations of a given image as positive samples for that image and other randomly chosen images in the batch as negative samples. Positive samples are pulled close together in representation space; and negative samples are pushed apart. MoCo-v2 \citep{chen2020improved} is an improved version of MoCo inspired by SimCLR \citep{chen2020simple}; key improvements are the addition of MLP projection heads and additional data augmentation such as Gaussian blurring. Nevertheless, scene cropping is still the most important augmentation. BYOL \citep{grill2020bootstrap} is an SSL approach that also uses data augmentation of an image as positive samples for that image. Positive samples are pulled close together in representation space. BYOL does not rely on negative samples (and hence is not contrastive). Instead, several other regularization techniques are required to prevent collapse to a trivial solution \citep{richemond2020byol}. 

We pretrain several SSL methods MoCo-v2, CMC \citep{tian2019contrastive}, SwAV  \citep{NEURIPS2020_70feb62b} and BYOL \citep{grill2020bootstrap} on our OpenImages dataset. 
MoCo-v2, BYOL, and other recent state of the art SSL approaches all relying on \emph{scene-scene} cropping of the same image to generate positive samples. This cropping strategy has also been used as a default data augmentation in supervised learning \citep{He2015,NIPS2012_c399862d,cubuk2019autoaugment}. The most common workflow is: choose a random scale (default range $0.2$ to $1.0$) and a random aspect ratio (default range $0.75$ to $1.33$). A crop is made from the original image using these two values (scale and aspect ratio). Finally, the crop is resized to the final size of $224 \times 224$ pixels. %This approach works well in the case of ImageNet where one object primarily occupies most of the area in an image. However, problems are encountered when applying this to the OpenImages dataset (see Fig \ref{fig:imagenet_openimages_figure} in supplementary).

We use a ResNet-50 \citep{He2015} deep network as the backbone for all experiments. After pre-training, we freeze the backbone weights, and train a linear classifier or fine-tune on the downstream datasets and tasks. We also train a randomly initialized ResNet-50 network in a fully supervised manner using ground truth labels and a multi-class logistic regression loss. We follow the mAP metric as described in section 4.2 of paper\citep{veit2017learning} (Eqn.(4)). Table \ref{tab:ssl_comparison_classification} shows our results. We see a significant difference in performance between fully supervised training and SSL approaches on the OpenImages dataset, with a gap of $16.3$ mAP points on average across the $4$ SSL approaches considered. On ImageNet, the top-1 accuracy gap is considerably smaller with an average gap of only $8.5$, nearly half that of OpenImages. The last row shows the significant boost obtained by using our object-aware cropping approach, which we describe in the next section, with MOCO-v2. The gap between SSL and supervised training on OpenImages is now the same as ImageNet.
% On ImageNet, where a single object tends to dominate the image, \emph{scene-scene} and \emph{obj-obj+dilate} perform at par.
\begin{table*}
    \centering
    \begin{tabu} to \linewidth {lcccc} 
        \toprule
        Model & OpenImages (mAP) & ImageNet (Top-1 $\%$)\\
         \midrule
         Supervised Performance & 66.3 & 76.2 \\ 
         \midrule
    %   CMC \citep{Tian2020ContrastiveMC} & 48.7(\color{red}{-17.6) & 60.0 (\color{red}{-16.2})\\
       CMC \citep{tian2019contrastive}  & 48.7 (\color{red}{-17.6}) & 60.0  ({\color{red}{-16.2}})\\
       BYOL \citep{grill2020bootstrap} & 50.2 (\color{red}{-16.1}) & 70.7  ({\color{red}{-5.5}})\\
       SwAV \citep{NEURIPS2020_70feb62b} & 51.3 (\color{red}{-15.0}) & 72.7 ({\color{red}{-3.5}})\\
       MoCo-v2 (Scene-Scene crop) & 49.8 (\color{red}{-16.5}) & 67.5  ({\color{red}{-8.7}})\\
        \midrule
        MoCo-v2 (Object-Object+Dilate crop) (Ours)  & 58.6 (\color{red}{-7.7}) & 68.0 ({\color{red}{-8.2}})\\
        \bottomrule
    \end{tabu}
    \vspace{0.1in}
    \caption{Classification results on OpenImages and Imagenet. For each SSL method, we show in parentheses the gap to fully supervised training (same number of epochs). The last row shows that our proposed approach using \emph{obj-obj+dilate} cropping reduces the gap on OpenImages by nearly half compared to the baselines, improving over the \emph{scene-scene} cropping based SSL methods by between $6.8$ to $9.4$ mAP points. We also observe improvements on ImageNet as well. }
    \label{tab:ssl_comparison_classification}
\end{table*}

\subsection{Analysis and Motivation}
We conduct further experiments to analyze better the results seen in Table \ref{tab:ssl_comparison_classification}, and to motivate our proposed approach. Our experiments help to narrow down scene cropping as one main cause of the poor performance of SSL on OpenImages, rather than other differences with ImageNet, such as object size, class distributions or image resolution.


\textbf{Object Size:} We compare MoCo-v2 performance to that of fully supervised learning, with both methods using scene-based cropping. Fig. \ref{fig:issue_scale_long_tail} (left) shows that the performance gap between supervised learning and SSL methods does not vary significantly for objects of different sizes in OpenImages. This suggests that once object sizes are below a threshold where scene cropping tends to ignore object information, MoCo-v2 performance is mostly independent of object scale. 

\textbf{Long-tail Distribution:} Even after selecting at least $900$ images per class, our OpenImages subset has a significant variation in the number of images per class (from around $1000$ to $60000$). Fig. \ref{fig:issue_scale_long_tail} (right) plots the performance of MoCo-v2 and supervised training as a function of the number of instances in each class. We do not see a significant change in relative performance as the number of instances in a class changes. This rules out long tails of the distribution as a cause for the poor absolute performance of MoCo-v2 on OpenImages.

% \vspace{-1.4in}
\begin{figure*}[t!]
  \centering
  \begin{subfigure}[t]{0.48\textwidth}
   \centering
    \includegraphics[width=\linewidth]{LaTeX/Images/map_for_each_class_and_sum_of_pixels_for_sup_and_moco_plotly_1.png}
   
    % \caption{ }
     \label{fig:scale_issue}
  \end{subfigure} 
  ~
  \begin{subfigure}[t]{0.48\linewidth}
   \centering
    \includegraphics[width=\linewidth]{LaTeX/Images/map_for_each_class_and_instances_for_sup_and_moco_plotly_1.png}
    % \caption{}
  \label{fig:long_tail_issue}
  \end{subfigure}
  \vspace{-0.3in}
    \caption{Analysis of OpenImages data distribution. Left: Performance of supervised and MoCo-v2 pre-training as a function of the scale of the objects; we plot the log of average of pixels against the sum of AP for each class. We see no discernible pattern of performance of MoCo-v2 or supervised learning as a function of object scale. Right: Performance of supervised learning and MoCo-v2 as a function of the number of instances in a class; we plot the log number of instances in a class against the sum of AP for that class. We do not see any discernible pattern of performance difference as a function of class size. \vspace{-10pt}}
\label{fig:issue_scale_long_tail}
\end{figure*}
% \vspace{-0.4in}
% Our OpenImages dataset is smaller than ImageNet by a factor of $5$. To confirm that dataset size is not the problem for SSL approaches,
\textbf{Can ImageNet pre-training help?}
 We pre-trained a supervised model on ImageNet and then fine-tuned the final fully-connected layer on the OpenImages dataset. We can see from the second column in Table  \ref{tab:openimages_analysis} that this pre-training does not help to close the performance gap. One of the reasons that ImageNet pre-training does not help is that OpenImages and ImageNet have significantly different class distributions (e.g. see \cite{li2019analysis} for a detailed analysis). %ImageNet has single large objects, whereas OpenImages has many small objects per image. 
 
\textbf{Can resizing the images help?}
We also experimented with resizing the images in OpenImages to the same approximate size ($384 \times 384$) and aspect ratio as ImageNet. The result is shown in the third column of Table \ref{tab:openimages_analysis} confirming that controlling for image size does not help to close the gap. 

\textbf{Can cropping on ground truth objects help?} 
%We use ground truth boxes for random cropping.  We can see from col $4$ that using ground truth boxes also doesn't help reduce the performance gap.
We see from column 4 of Table \ref{tab:openimages_analysis} that using random cropping on ground truth object boxes does not help reduce the performance gap either. As we show later in Section\ref{sec:model} that learning from both object and context is important for learning semantic information on multi-object datasets. 

\textbf{Varying the lower scale of random resized crop:}  MoCo-v2 (\cite{chen2020improved}) used scene crops whose size was chosen from a uniform distribution ranging from $20\%$ to $100\%$ of the ImageNet image size ($384 \times 384$). Since OpenImages images are bigger and objects generally occupy a smaller fraction compared to ImageNet, we vary the lower bound for scene crops to measure the impact. The last six columns of Table \ref{tab:openimages_analysis} shows that varying the range of scene crop is insufficient to close the performance gap. 

We conclude that the performance gap between supervised training and SSL training is likely due to the data augmentation, rather than characteristics of the image distribution. Further analysis experiments are provided in the supplementary (Sec \ref{sec:analysis_openimages_more}). 

% This shows that network is still not able to capture the smaller objects in the image doesn't really help in achieving good performance. \\

% \vspace{-5pt}
% \begin{wraptable}{r}{5.5cm}
% \vspace{-30pt}
% \begin{table*}
%     \centering
%     \begin{tabu} to \linewidth {lccc} 
%         \toprule
%         Model & mAP (Classification) \\
%          \midrule
%          Supervised OpenImages & 66.3
%         \\ 
%          \midrule
%       %Ground truth object crops & 22.8 \\
%       MoCo-v2: Pretraining on ImageNet & 28.3 \\
      
%         MoCo-v2: Resizing all images to ImageNet size ($384 \times 384$) & 45.9 \\
%          MoCo-v2: Cropping on ground-truth objects & 45.3 \\
%       MoCo-v2: scene crop range $0.8$-$1.0$ & 26.5 \\
%       MoCo-v2: scene crop range $0.6$-$1.0$ & 37.6 \\
%       MoCo-v2: scene crop range $0.4$-$1.0$ & 45.6 \\
%       MoCo-v2: scene crop range $0.2$-$1.0$ & 49.8 \\
%       MoCo-v2: scene crop range $0.1$-$1.0$ & 46.1 \\
%       MoCo-v2: scene crop range $0.05$-$1.0$ & 43.1 \\
%         \bottomrule
%     \end{tabu}
%     \vspace{0.1in}
%     \caption{Linear evaluation on our OpenImages dataset with different pre-training strategies with MoCo-v2 (see Section \ref{sec:analysis} for details). The top row uses fully supervised learning on OpenImages. We see that for self-supervised pre-training, no specific range of scene crops helps to close the large gap between SSL and supervised training. However, there is a sweet spot of scene crop range where MoCo-v2 performance is highest. \vspace{-20pt}}
%     % \vspace{-1.5ex}
%     \label{tab:openimages_analysis}
% \end{table*}

\begin{table*}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabu} to \linewidth {cccc|cccccc} 
        \toprule
        &IN&Resize to &&\multicolumn{6}{c}{Scene-Scene Crop} \\
        Supervised & Pretraining & ($384 \times 384$) & GT-Crop & 0.8-1.0 &  0.6-1.0 & 0.4-1.0 & 0.2-1.0 & 0.1-1.0 & 0.05-1.0 \\
         \midrule
         66.3 & 28.3 & 45.9 & 45.3 & 26.5 & 37.6 & 45.6 & 49.8 & 46.1 & 43.1 \\
    %     \\ 
    %      \midrule
    %   %Ground truth object crops & 22.8 \\
    %   MoCo-v2: Pretraining on ImageNet & 28.3 \\
      
    %     MoCo-v2: Resizing all images to ImageNet size ($384 \times 384$) & 45.9 \\
    %      MoCo-v2: Cropping on ground-truth objects & 45.3 \\
    %   MoCo-v2: scene crop range $0.8$-$1.0$ & 26.5 \\
    %   MoCo-v2: scene crop range $0.6$-$1.0$ & 37.6 \\
    %   MoCo-v2: scene crop range $0.4$-$1.0$ & 45.6 \\
    %   MoCo-v2: scene crop range $0.2$-$1.0$ & 49.8 \\
    %   MoCo-v2: scene crop range $0.1$-$1.0$ & 46.1 \\
    %   MoCo-v2: scene crop range $0.05$-$1.0$ & 43.1 \\
        \bottomrule
    \end{tabu}}
    %\vspace{0.1in}
    \caption{Linear evaluation on our OpenImages dataset with different pre-training strategies with MoCo-v2 (see Section \ref{sec:analysis} for details). Column 1 uses fully supervised learning on OpenImages. We see that for self-supervised pre-training, no specific range of scene crops helps to close the large gap between SSL and supervised training. However, there is a sweet spot of scene crop range where MoCo-v2 performance is highest.} %\vspace{-20pt}}
    % \vspace{-1.5ex}
    \label{tab:openimages_analysis}
\end{table*}



% \end{wraptable}

==> LaTeX/Images/related.tex <==
\section{Related Work}
\vspace{-5pt}
\label{secc:related}
% In this section we review the relevant methods Self-Supervised and contrastive learning methods. We will also discuss the methods that discuss the importance of data augmentations in SSL methods.  
Recent progress in self-supervised learning, based on contrastive and non-contrastive approaches, has achieved excellent performance on various domains, datasets and tasks \citep{he2019momentum,chen2020improved,chen2020simple,Oord2018RepresentationLW,tian2019contrastive,gidaris2020learning,misra2019selfsupervised,NEURIPS2020_4c2e5eaa,8578491,grill2020bootstrap,Gidaris2018UnsupervisedRL,Larsson2017ColorizationAA,Noroozi_2018_CVPR,Pathak2016ContextEF}. The top-performing methods have all used related ideas of pulling together ``views" of a sample in representation space. Some of these approaches, in addition, use negative samples to add a ``push" factor, and this is termed contrastive self-supervised learning. Theoretical and empirical studies have been published to better understand the behavior and limitations of these approaches  \citep{arora2019theoretical,xiao2021contrastive,purushwalkam2020demystifying,tosh2021contrastive,wang2020understanding,yang2020xlnet,NEURIPS2020_63c3ddcc,liu2021selfsupervised,kalantidis2020hard,Newell_2020,cai2020negatives}. 

A number of papers have observed that the default SSL approaches above (whether contrastive or not) perform poorly on uncurated datasets such as OpenImages \citep{kuznetsova2020open}. To address this, recent works have used different workarounds such as knowledge distillation \citep{tian2021divide}, clustering \citep{goyal2021selfsupervised}, localization \citep{selvaraju2020casting}, unsupervised semantic segmentation masks \citep{henaff2021efficient}, pixel-level pretext tasks\citep{xie2021propagate}, Instance localization \citep{yang2021instance} and local contrastive learning \citep{liu2021selfemd}. The common element among top-performing image-based SSL approaches, regardless of dataset, task or architecture, is their reliance on strong data augmentations such as random cropping, gaussian blurring, color jittering or rotations. These augmentations create meaningful positive views, and other randomly sampled images in the dataset are used to create negative views in the case of contrastive SSL methods. SSL data augmentation pipelines are adapted from the supervised learning literature \citep{cubuk2019autoaugment,zoph2020rethinking,NIPS2012_c399862d,2003aug,devries2017dataset,cubuk2019autoaugment,zhang2018mixup,cubuk2019randaugment,wu2019detectron2,yun2019cutmix,lim2019fast,hataya2019faster}.

The closest work to our object cropping work is \citep{selvaraju2020casting}, which introduces a technique to choose crops around objects based on saliency maps \citep{Selvaraju2016GradCAMVE}, showing good improvements over the baseline of random crops for COCO datasets (see Table \ref{tab:coco_detection}). As shown in our results, Obj-Obj+Dilate crop consistently performs better than \citep{selvaraju2020casting} (Table \ref{tab:coco_detection}). Our approach is also significantly simpler to incorporate into existing pipelines, requiring no change to the training, architecture or loss. \citet{vangansbeke2021revisiting} show that constrained multi-cropping improves performance of SSL methods: our approach can be incorporated into their pipeline to further improve performance. 

%A fundamental underlying assumption in these methods is the fact that these datasets are object centred, i.e a single object occupies most of the image. This assumption holds true for ImageNet but it doesn't hold true for OpenImages dataset \citep{Kuznetsova_2020}. In our work we show that by using BING crops we can focus more on object centric features which transfer well. Another recently famous line of work that has gained lot of popularity in the recent times doesn't use negative samples \citep{grill2020bootstrap,caron2021unsupervised,Caron2020UnsupervisedLO,chen2020exploring}. We show the efficacy of our method on both of these types of contrastive learning approaches and significantly improve  upon the baseline methods.



% Divide and Contrast \citep{tian2021divide} firstly uses clustering to build semantically  meaningful clusters from the uncurated datasets and then uses teacher network using knowledge distillation to further improve the representations.
% CASTing model \citep{selvaraju2020casting} uses Grad-CAM to detect objects and improve performane on "non-iconoic" datasets. DetCon \citep{henaff2021efficient} uses unsupervised semantic segmentation masks to localize objects and uses object from the same mask as positive samples. However unlike DetCon \citep{henaff2021efficient}  we use Objectness predicting algorithms and also entanglement of object and scene crops. Sel-EMD \citep{liu2021selfemd} uses Earth Mover's Distance between the features of an image and tries to learn features from relevant and overlapping image region between two crops.  

% Learning from uncurated datasets is one of the most fundamental problems in SSL. Many recent works have tried to address and solve the problem of leaning from uncurated datasets. Divide and Contrast \citep{tian2021divide} firstly uses clustering to build semantically  meaningful clusters from the uncurated datasets and then uses teacher network using knowledge distillation to further improve the representations.
% CASTing model \citep{selvaraju2020casting} uses Grad-CAM to detect objects and improve performane on "non-iconoic" datasets. DetCon \citep{henaff2021efficient} uses unsupervised semantic segmentation masks to localize objects and uses object from the same mask as positive samples. However unlike DetCon \citep{henaff2021efficient}  we use Objectness predicting algorithms and also entanglement of object and scene crops. Sel-EMD \citep{liu2021selfemd} uses Earth Mover's Distance between the features of an image and tries to learn features from relevant and overlapping image region between two crops. Our proposed method however is complementary to these approaches and can potentially be augmented with any of these methods. 

% These methods show improved results across various datasets like ImageNet \citep{imagenet_cvpr09}, Stanford Cars \citep{KrauseStarkDengFei-Fei_3DRR2013}, CIFAR \citep{cifar}, SVHN \citep{goodfellow2014multidigit}.  MixUp \citep{zhang2018mixup}. 
 
% AutoAugment  \citep{cubuk2019autoaugment} uses Reinforcement Learning to search for improved data augmentations policies. They show improved results across various datasets like ImageNet \citep{imagenet_cvpr09}, Stanford Cars \citep{KrauseStarkDengFei-Fei_3DRR2013}, CIFAR \citep{cifar}, SVHN \citep{goodfellow2014multidigit}.  MixUp \citep{zhang2018mixup} trains a neural network on convex combinations of examples and their labels. MixUp forces the neural networks to behave linearly between training samples. RandAug \citep{cubuk2019randaugment} is another data augmentation similar to AutoAugement which uses significantly less search space and can achieves state-of-art results across various datasets. However one of the issues in these methods is use of Random Cropping which we have shown doesn't work well in case of multi-object datasets. 

% \textbf{Importance of cropping vs other data augmentations:} Random Crop augmentation has been central to achieving state-of-the art results in SSL \citep{chen2020simple}(see Fig5). GLOM \citep{Hinton2021HowTR} also discusses the importance of having scene level representations vs object level representations for building all purpose models such as GLOM \citep{Hinton2021HowTR}. GLOM touches upon the idea that contrastive learning on non-iconic datasets will not work well due to the presence of multiple objects. To solve this problem we have proposed using both object level and scene level representations in conjunction with each other. We also analyze various other possibilities such as using object-object, object-scene and scene-scene representations and discuss the various other factors that could impact the performance. However we find that simple object-scene level cropping shows best performance for non-iconic datasets.    

==> LaTeX/Images/results.tex <==
%\vspace{-0.15in}
\section{Results}
\label{secc:results}
%\subsection{Datasets}
% We begin by describing OpenImages-Subset datset followed by COCO and ImageNet.
% \subsubsection{OpenImages Dataset}
%\label{sec:openimages_dataset}
% OpenImages has a total of 9.1 million images present in the dataset, however we are only focusing on the subset of OpenImages which has labelled bounding boxes. This smaller subset of OpenImages has close to 1.9 million images. However unlike ImageNet this subset is unbalanced and has a distribution with a long tail. To remove this long-tail and unbalanced distribution we create a balanced subset of OpenImages. To achieve this we use a greedy algorithm: \\
% \begin{itemize}
% \vspace{-0.2in}
% \item Protocol1 - We only select the images which have at least 2 or more classes present in the image. This brings down the total number of images from 1.9 million to close to 1.1 million.

% \item  Protocol2 - Now we only select the classes which have minimum of 900 images present in them. 
% After setting 900 as the low\_threshold, the number of classes selected were 208 and the number of images selected are 212753. 
% \end{itemize}
%\vspace{-0.15in}
\begin{table*}
    \centering
    \begin{tabu} to \linewidth {lccccc} 
        \toprule
        Model & Crops & Obj-Obj+Dilate & Obj-Scene & Scene-Scene  & mAP \\
        
         \midrule
          
         Supervised  & - & - & - & -  &  66.3 \\ 
         \midrule
         MoCo-v2 & Ground Truth boxes & -  & \Checkmark & - &  58.9\\ 
         
         MoCo-v2 & Ground Truth boxes &  \Checkmark   & - & - &  60.2\\ 
         \midrule
     MoCo-v2  &- & - & - & \Checkmark &  49.8\\
      BYOL & -   & - & - & \Checkmark &  50.2 \\
      \midrule
         % MoCo-V2( BING crops)  & _ & \checkmark & _ & _ & 58.1\\
       
      
    % MoCo-v2  & -  & \Checkmark & -  & - &  54.1\\
    
    % 
    %  \midrule
%     MoCo-V2 using object and object crops  &  100 & 54.1\\
%      \midrule
    
    %  MoCo-V2  & \Checkmark & \Checkmark  & \Checkmark &  80 - 100 & 55.7\\    
    %  MoCo-v2 ( Radius: 100 - 120 )  & \Checkmark & \Checkmark  & \Checkmark &   57.1\\  
    %  MoCo-V2  & \Checkmark & \Checkmark  & \Checkmark &  120 - 140 & 53.2\\  
    %  MoCo-V2  & \Checkmark & \Checkmark  & \Checkmark & 160 - 180 & 52.3\\  
    %  MoCo-V2  & \Checkmark & \Checkmark  & \Checkmark &  180 - 200 & 51.8\\  
    %   MoCo-V2  & \Checkmark & \Checkmark  & \Checkmark & 200 - 240 & 50.9\\  
%     MoCo-V2  combining all three methods &  100 - 120 & 57.1\\
%  MoCo-V2 combining all three methods &  120 - 140 & 52.8\\
%     MoCo-V2 combining all three methods &  140 - 160 & _\\
%     MoCo-V2 combining all three methods &  160 - 180 & 51.8\\
%     MoCo-V2 combining all three methods &  180 - 200 & 51.2\\
%      MoCo-V2 combining all three methods &  200 - 240 & 51.5\\
 %\midrule
 
 MoCo-v2 & Unsupervised proposal boxes & - & \Checkmark & - &  58.0\\ 
 MoCo-v2 & EdgeBoxes crops & - & \Checkmark  & - &  57.1\\
    MoCo-v2 & BING crops   & - & \Checkmark & - &  58.1 \\   
    
     BYOL & BING crops   & - & \Checkmark & - &  58.5 \\
     \midrule
     MoCo-v2 &BING crops & \Checkmark   & -  & - &  58.6\\
    BYOL & BING crops & \Checkmark  & -  & - &  59.1\\
     
     
        \bottomrule
    \end{tabu}
    \vspace{-0.05in}    
  \caption{Crop approaches on OpenImages: using BING crops to generate one view, and a dilated crop or a scene crop for the other positive, we are able to reduce the difference between SSL and Supervised Learning by close to $50\%$ (compare the last two rows to the first row). Using ground-truth boxes to generate crops from OpenImages improves the pre-training performance marginally compared to BING crops. Obj-Obj+Dilate (last two rows) have the best performance, although Obj-Scene also does well compared to Scene-Scene.}  
  \label{tab:openimages_moco}    
\end{table*}
% this table is confusing.  First, why is, say Obj-Scene its own column, while Object-Dilated is a type of crop?  Why is BYOL not done with Object-Dilated or Obj-Obj+Shift?  But mostly you are doing very different things all mixed together.  On the one hand, you are comparing different types of proposals.  But you are also comparing different kinds of cropping strategies.  The most important point, that a good cropping strategy improves greatly over scene-scene gets kind of lost.  It would be better probably to separate this into different tables.  Also, the Ground Truth boxes are not a real method, instead it's a kind of upper bound on the others, but the structure of the table doesn't make this clear.  Also, Object-Dilated is using a Bing crop, right?  But it explicitly doesn't say BING crop. I think from this table that dilated works only marginally better than object-scene.  In that case, in the previous section, these should be presented as two similar approaches.

% I think from this table that dilated works only marginally better than object-scene.  In that case, in the previous section, these should be presented as two similar approaches.

We created a subset of the OpenImages dataset with $212$k images, as described in Section \ref{sec:analysis}. We also experiment with the complete OpenImages ($\sim$1.9 million images.)
% Each image in this dataset (which we still refer to as OpenImages) has on an average $12$ objects present. Further details of this dataset are provided in the Supplementary material in Sec \ref{sec:details_openimages}. 
In addition, we perform pre-training on ImageNet \citep{imagenet_cvpr09} and MS-COCO \citep{Lin2014MicrosoftCC}.
ImageNet (with $1.2$M training images) has been extensively used and is the standard dataset used for benchmarking of SSL methods. MS-COCO has $\sim118$k training images and $896$k labelled objects which is approximately $7$ objects per image. For pre-training on MoCo-v2, we closely follow the standard protocol described in \citet{chen2020improved}. We randomly select from $10$ object proposals provided by BING, Edge-Boxes or the unsupervised proposal method of \citep{vo2019unsupervised}. All our training and evaluation is performed on a ResNet-50 \citep{He2015}. 

% However, our main focus is non-iconic datasets like MS-COCO and OpenImages, so we only experiment using the ImageNet-100 dataset, which has been used in recent works like Info-Min \citep{tian2020contrastive}.

We evaluate the pre-trained models on classification (linear evaluation), object detection and semantic segmentation. For VOC object detection, COCO object detection and COCO semantic segmentation, we closely follow the common protocols listed in Detectron2 \citep{wu2019detectron2}. For VOC object detection, we evaluate on the Faster-RCNN(C4-backbone) \citep{Ren2015FasterRT} detector on VOC \texttt{trainval07+12} dataset  using the standard 1 $\times$  standard protocol. For COCO-Object detection and semantic segmentation, we fine tune on the MaskRCNN detector (FPN-backbone) \citep{he2018mask} on COCO \texttt{train2017} split ($118$k images) with the standard 1 $\times$ schedule, evaluating on the COCO 5k \texttt{val2017 split}. We compare to the state of the art SSL methods, including Self-EMD \citep{liu2021selfemd}, DetCon \citep{henaff2021efficient}, BYOL \citep{richemond2020byol}, DenseCL \citep{wang2021dense} and the default MoCo-v2 \citep{chen2020improved}. 
% Our method can also be used with more recent SSL methods such as DenseCL \citep{wang2021dense} (concurrent work to ours).


%Note that we compare most of our results with Self-EMD \citep{liu2021selfemd} and DetCon \citep{henaff2021efficient}, and not with DenseCL \citep{wang2021dense} since they use different hyper-parameter settings than the standard ones present in MoCo-v2 \citep{he2019momentum}. Moreover, our aim is to present a generic method of data augmentation that can be fitted into any of these pipelines and improve these methods.   \\

%% Move to supplementary
%We use a learning rate $0.03$, weight decay of $0.0001$ and momentum of $0.9$. We train on $4$-GPUs with a mini batch-size of $256$ for $800$ epochs. 



%% move to supplementary 
%For linear evaluation, we closely follow MoCo-V2 and use Learning-Rate(LR) of 30 using an SGD optimizer. 




\begin{table*}
    \centering
    \begin{tabu} to \linewidth {lcccccc} 
        \toprule
        % Description & AP & AP_{50} & AP_{75} &AP_{s} & AP_{l} & AP_{m} \\
        Description & $AP$ & $AP_{50}$ & $AP_{75}$ & $AP_{s}$ & $AP_{l}$ & $AP_{m}$ \\
         \midrule
    %   MoCo-V2 \cite{He2020MomentumCF}  & 50.86 & 77.60&55.43\\
    %     MoCo-V2 using object and context crops (Ours)  & 52.91 & 79.61 & 57.96\\
    Supervised (Random Initialization) & 32.8 & 50.9 & 35.3 & 29.9 & 47.9 & 32.0 \\
    Supervised (ImageNet Pre-trained) & 39.7 & 59.5 & 43.3 & 35.9 & 56.6 & 38.6 \\
     \midrule
    MoCo-v2 \citep{chen2020improved}  & 38.2 & 58.9 & 41.6 & 34.8 & 55.3 & 37.8\\
    BYOL \citep{henaff2021efficient}  & 38.8 & 58.5 & 42.2 & 35.0 & 55.9& 38.1\\
    Dense-CL \citep{wang2021dense} & 39.6 & 59.3 & 43.3 & 35.7 & 56.5 & 38.4 \\
    CAST \citep{selvaraju2020casting} (180K steps) & 39.4 &  60.0 & 42.8 & 35.8 & 57.1 & 37.6 \\ 
    Self-EMD \citep{liu2021selfemd} (Uses BYOL)  & 39.8 & 60.0 & 43.4 & - & -& -\\
    \midrule
    MoCo-V2 (Obj-Scene) (Ours)  & 39.4 & 59.8 & 42.9 & 35.8 & 57.8 & 38.7\\
     
   
    % MoCo-v2 - All-three-crops (Ours)  & \cellcolor{blue!15}\textbf{39.7} & \cellcolor{blue!15}\textbf{60.1} & \cellcolor{blue!15}\textbf{43.4} & \cellcolor{blue!15}\textbf{36.0} & \cellcolor{blue!15}\textbf{57.3} & \cellcolor{blue!15}\textbf{38.6}\\
    % MoCo-v2 - All-three-crops (180K steps) (Ours)  & \cellcolor{blue!15}\textbf{40.2} & \cellcolor{blue!15}\textbf{60.6} & \cellcolor{blue!15}\textbf{43.6} & \cellcolor{blue!15}\textbf{36.3} & \cellcolor{blue!15}\textbf{57.4} & \cellcolor{blue!15}\textbf{39.0}\\
    
    MoCo-v2 (Obj-Obj+Dilate) (Ours)  & \cellcolor{blue!15}\textbf{39.7} & \cellcolor{blue!15}\textbf{60.1} & \cellcolor{blue!15}\textbf{43.4} & \cellcolor{blue!15}\textbf{36.0} & \cellcolor{blue!15}\textbf{57.3} & \cellcolor{blue!15}\textbf{38.8}\\
    MoCo-v2 (Obj-Obj+Dilate) (180k steps)  & \cellcolor{blue!15}\textbf{40.2} & \cellcolor{blue!15}\textbf{60.6} & \cellcolor{blue!15}\textbf{43.6} & \cellcolor{blue!15}\textbf{36.3} & \cellcolor{blue!15}\textbf{57.4} & \cellcolor{blue!15}\textbf{39.0}\\
    \midrule
     BYOL (Obj-Obj+Dilate) (Ours)  & \cellcolor{blue!15} \textbf{40.1} & \cellcolor{blue!15} \textbf{60.8} & \cellcolor{blue!15} \textbf{43.6} & \cellcolor{blue!15} \textbf{36.4} & \cellcolor{blue!15} \textbf{58.4} & \cellcolor{blue!15} \textbf{39.5}\\
      
     Dense-CL (Obj-Obj+Dilate) (Ours)  & \cellcolor{blue!15}\textbf{40.4} & \cellcolor{blue!15}\textbf{60.4} & \cellcolor{blue!15}\textbf{44.0} & \cellcolor{blue!15}\textbf{36.6} & \cellcolor{blue!15}\textbf{57.9} & \cellcolor{blue!15}\textbf{39.5}\\
     
        \bottomrule
    \end{tabu}
    \caption{Object detection (first 3 columns) and Semantic Segmentation (last 3 columns) results on COCO dataset. All SSL models have been pre-trained on COCO dataset and then finetuned on COCO. Note that for the same number of finetuning iterations ($180$K), we outperform CAST \citep{selvaraju2020casting} which also relies on localized crops. All other methods are run for $90$K, finetuning iterations. For any SSL method, we compare (BYOL, Moco-v2, Dense-CL) adding Obj-Obj+Dilate crop improves performance.}
    \label{tab:coco_detection}
\end{table*}



\begin{table*}
    \centering
    \begin{tabu} to \linewidth {lcccccc} 
        \toprule
        % Description & AP & AP_{50} & AP_{75} &AP_{s} & AP_{l} & AP_{m} \\
        Description & $AP$ & $AP_{50}$ & $AP_{75}$ & $AP_{s}$ & $AP_{l}$ & $AP_{m}$ \\
        
    %   MoCo-V2 \cite{He2020MomentumCF}  & 50.86 & 77.60&55.43\\
    %     MoCo-V2 using object and context crops (Ours)  & 52.91 & 79.61 & 57.96\\
    
     \midrule
    COCO: MoCo-v2 (Scene-Scene crop) & 38.2 & 58.9 & 41.6 & 34.8 & 55.3 & 37.8\\
    
   
   
    COCO: MoCo-v2 (Obj-Obj+Dilate crop)  & \cellcolor{blue!15}\textbf{40.2} & \cellcolor{blue!15}\textbf{60.6} & \cellcolor{blue!15}\textbf{43.6} & \cellcolor{blue!15}\textbf{36.3} & \cellcolor{blue!15}\textbf{57.4} & \cellcolor{blue!15}\textbf{39.0}\\
    \midrule
    VOC: MoCo-v2 (Scene-Scene crop) & 56.1 & 81.3 & 61.3 & - & - & -\\
    VOC: MoCo-v2 (Obj-Obj+Dilate crop)  & \cellcolor{blue!15} \textbf{57.6} & \cellcolor{blue!15} \textbf{82.5} & \cellcolor{blue!15}\textbf{63.8} & - & - & -\\
        \bottomrule
    \end{tabu}
    \caption{Object detection (first 3 columns) and semantic segmentation (last 3 columns) results on COCO (first 2 rows) and VOC (last 2 rows). All SSL models have been pre-trained on complete OpenImages dataset(1.9 million images) for 75 epochs and then finetuned on COCO and VOC dataset.}
    \label{tab:openimages_full_results}
\end{table*}

%\subsection{Results}
Table \ref{tab:ssl_comparison_classification} and Table \ref{tab:openimages_moco} shows results on OpenImages dataset. We perform ablation studies on $3$ different types of crops. We can see that the best performing Obj-Obj+Dilate crops outperform the baseline by $8.2$ mAP, closing the gap between supervised learning and MoCo-v2 baseline by almost $50\%$. Obj-Scene crops also outperform the baseline by $8.1$ mAP.  Obj-Obj+Shift crops ($54.1$ mAP) do not perform as well as Obj-Obj+Dilate or Obj-Scene. We believe this is because the second object crop is chosen at a certain minimum radius from the first (otherwise, the overlap between the crops is too large to produce meaningful learning). The second object crop, therefore, contains only part of the object. Conversely, a dilated object crop would potentially contain the entire object and more scene information; therefore, the representation from the dilated object-crop contains complementary information from both the object and the scene. 
% Combining all three cropping methods works slightly worse than simply using object-scene crops for OpenImages. 
We also show in Table \ref{tab:openimages_moco} an ablation with ground truth bounding boxes being used to guide the object cropping. This performs marginally better than the use of BING crops, suggesting that a tight fit around the object is not necessary for improved representations. 

% We also perform Transfer learning experiments on VOC dataset using OpenImages pre-training (present in the supplementary materials). Even in the transfer learning setup Object-Scene crops and Dilated-Object crops perform better than Object-Object crops.


% Finally, in Table \ref{tab:ssl_comparison_classification}, we show results on ImageNet. Since objects in ImageNet are large and centered, we expect object-scene cropping to perform at par with scene-scene cropping. This is indeed the case: object-scene crop performs better by a small margin of $0.1\%$ in top-1 accuracy.

% add back this line if we show dilated 
%One of the reason this could be that BING not only gives object proposals it also introduces some extra context. This extra context might be helping the SSL methods produce representations which work well. \\

Table  \ref{tab:coco_detection} shows results on object detection and semantic segmentation for COCO (by pre-training on COCO \texttt{trainval2017} datasets and finetuning on COCO). We train MoCo-v2 and BYOL models. Our MoCo-v2 Obj-Obj+Dilate cropping outperforms MoCo-v2 Scene-Scene baseline and Obj-Scene cropping. For semantic segmentation, we outperform the MoCo-v2 baseline. Our proposed cropping is agnostic to the pre-training SSL method; we show state-of-art results by adding our approach to Dense-CL \citep{wang2021dense}. We also outperform the CAST model \citep{selvaraju2020casting} which also uses localized crops based on saliency maps: our approach is simpler and performs better by around $0.5$ mAP. Table \ref{tab:voc_moco} (supplementary) shows results of object detection on PASCAL-VOC. We pre-train on COCO and then fine-tune on VOC. Obj-Obj+Dilate cropping outperforms the MoCo-v2 baseline by $3.2$ mAP; Obj-Scene cropping outperforms the MoCo-v2 baseline by $2.4$ mAP and the BYOL baseline by $2.5$ mAP. Improved results on iconic datasets like Aircraft, Birds and Cars can be found in Supplementary (Table~\ref{tab:object-object-analysis}). Additional results on varying number of proposals used can be found in Supplementary (Table~\ref{tab:voc_moco_proposals}). 

Table \ref{tab:openimages_full_results} shows results  on object detection and semantic segmentation for COCO and object-detection on VOC by pre-training on full OpenImages dataset \citep{kuznetsova2020open} (all 1.9 million images) for 75 epochs. We show improved performance over the baseline on both object detection and semantic segmentation tasks by using Obj-Obj+Dilate crops. Our proposed dilation method works not only for small multi-object datasets like COCO but also for datasets like OpenImages and performs well under a transfer learning setup.

{\textbf{Results on ImageNet:}} We also show improved results on ImageNet pre-training using object-aware cropping (Table~\ref{tab:imagenet_results} Supplementary) and MoCo-v2. For object detection on VOC2007, we see an improvement of 1.0 mAP; and a $0.5$ mAP improvements for object detection on COCO. Our approach is thus adaptable to the pre-training dataset and SSL algorithm. 


%The BING crop is close to $82\%$ of the image (on average). Therefore, we simply take standard random crops on the BING crops to generate both views. We then fine-tune our model on standard object detection task on VOC2007 and see an improvement of 1.0 mAP (Table~\ref{tab:imagenet_results} Supplementary). We also observe a $0.5$ mAP improvements for object detection on MS-COCO dataset with ImageNet pre-training. Small improvements on ImageNet can be attributed to the fact that ImageNet images contain a single object and hence random crops have very high chance of picking up objects.  


% \vspace{-5pt}

% We also show results on classification on the COCO dataset as shown in the Table \ref{tab:openimages_coco}. We can see that we improve by 5.2 MAP on COCO-Classification. 


% \begin{table*}
%     \centering
%     \begin{tabu} to \linewidth {lccc} 
%         \toprule
%         Description & radius & classification-map \\
%          \midrule
%          Supervised OpenImages & - & 66.3
%         \\ 
%          \midrule
%       MoCo-V2 \cite{He2020MomentumCF}  & - & 49.8\\
%      MoCo-V2  using random and ground-truth bounding boxes  & - & 58.2\\   
%     MoCo-V2  using random and BING crops  & - & 58.1\\
%      \midrule
%     MoCo-V2 using object and object crops  &  100 & 54.1\\
%      \midrule
%      MoCo-V2  combining all three methods &  80 - 100 & 55.7\\     
%     MoCo-V2  combining all three methods &  100 - 120 & 57.1\\
%  MoCo-V2 combining all three methods &  120 - 140 & 52.8\\
%     MoCo-V2 combining all three methods &  140 - 160 & _\\
%     MoCo-V2 combining all three methods &  160 - 180 & 51.8\\
%     MoCo-V2 combining all three methods &  180 - 200 & 51.2\\
%      MoCo-V2 combining all three methods &  200 - 240 & 51.5\\
%         \bottomrule
%     \end{tabu}
%   \caption{Classification results on OpenImages dataset.}  
%   \label{tab:openimages_moco}    
% \end{table*}






% \begin{table*}
%     \centering
%     \begin{tabu} to \linewidth {lccccc} 
%         \toprule
%         Method & Object-Object & Object-Scene & Scene-Scene & Radius & mAP \\
%          \midrule
%          Supervised OpenImages & - & - & - & - &  66.3 \\ 
%          \midrule
%      MoCo-v2 (Scene crops) & - & - & \Checkmark & - & 49.8\\
%          % MoCo-V2( BING crops)  & _ & \checkmark & _ & _ & 58.1\\
%     MoCo-v2( Edge crops) & - & \Checkmark  & - & - & 57.1\\
     
%     MoCo-v2 & \Checkmark  & -  & - & - & 54.1\\
%     % \midrule
%     %  \midrule
% %     MoCo-V2 using object and object crops  &  100 & 54.1\\
% %      \midrule
    
%     %  MoCo-V2  & \Checkmark & \Checkmark  & \Checkmark &  80 - 100 & 55.7\\    
%      MoCo-v2  & \Checkmark & \Checkmark  & \Checkmark &  100 - 120 & 57.1\\  
%     %  MoCo-V2  & \Checkmark & \Checkmark  & \Checkmark &  120 - 140 & 53.2\\  
%     %  MoCo-V2  & \Checkmark & \Checkmark  & \Checkmark & 160 - 180 & 52.3\\  
%     %  MoCo-V2  & \Checkmark & \Checkmark  & \Checkmark &  180 - 200 & 51.8\\  
%     %   MoCo-V2  & \Checkmark & \Checkmark  & \Checkmark & 200 - 240 & 50.9\\  
% %     MoCo-V2  combining all three methods &  100 - 120 & 57.1\\
% %  MoCo-V2 combining all three methods &  120 - 140 & 52.8\\
% %     MoCo-V2 combining all three methods &  140 - 160 & _\\
% %     MoCo-V2 combining all three methods &  160 - 180 & 51.8\\
% %     MoCo-V2 combining all three methods &  180 - 200 & 51.2\\
% %      MoCo-V2 combining all three methods &  200 - 240 & 51.5\\
%  %\midrule
%     MoCo-v2 (GT boxes) & - & \Checkmark & - & - & 58.2\\ 
%     MoCo-v2 (BING crops)   & - & \Checkmark & - & - & 58.1 \\   
%     BYOL (BING crops)   & - & \Checkmark & - & - & 58.5 \\
%         \bottomrule
%     \end{tabu}
%   \caption{Comparing different crop approaches on OpenImages: we show that by using BING crops to generate one positive, and a scene crop for the other positive, we are able to reduce the difference between SSL and Supervised Learning by close to $50\%$ (compare last two rows to first two rows). Using ground-truth boxes to generate crops from OpenImages improves the pre-training performance marginally compared to BING crops. Other combinations such as using object-object or all three crops underperform object-scene crops.}  
%   \label{tab:openimages_moco}    
% \end{table*}
% \begin{table*}
%     \centering
%     \begin{tabu} to \linewidth {lcccc} 
%         \toprule
%         Description & tau & AP & AP_{50} & AP_{75} \\
%          \midrule
%     %   MoCo-V2 \cite{He2020MomentumCF}  & 50.86 & 77.60&55.43\\
%     %     MoCo-V2 using object and context crops (Ours)  & 52.91 & 79.61 & 57.96\\
%     Supervised & - & 56.8 & 83.2 & 63.7 \\
%      \midrule
%     MoCo-V2 \cite{He2020MomentumCF}  & 0.2 & 50.8 & 77.6 & 55.4\\
%     \midrule
%     MoCo-V2 using object and context crops  & 0.2 & 54.0 & 79.9 & 59.1\\
%      MoCo-V2 using object and context crops  & 0.3 & 54.2 & 80.1 & 60.0\\
%      MoCo-V2 using object and context crops  & 0.4 & 54.1 & 80.0 & 60.0\\
%      MoCo-V2 using object and context crops  & 0.5 & 53.7 & 80.2 & 59.2\\ 
%         \bottomrule
%     \end{tabu}
%     \caption{Impact of varying tau. The models have been pre-trained on COCO dataset and then transferred to VOC.}
%     \label{tab:voc_analysis_tau}
% \end{table*}



% \begin{table*}
%     \centering
%     \begin{tabu} to \linewidth {lcccc} 
%         \toprule
%         Description & radius & AP & AP_{50} & AP_{75} \\
%          \midrule
%     %   MoCo-V2 \cite{He2020MomentumCF}  & 50.86 & 77.60&55.43\\
%     %     MoCo-V2 using object and context crops (Ours)  & 52.91 & 79.61 & 57.96\\
%     Supervised & - & 56.8 & 83.2 & 63.7 \\
%      \midrule
%     MoCo-V2 \cite{He2020MomentumCF}  & - & 50.8 & 77.6 & 55.4\\
%     \midrule
%     MoCo-V2 using object and context crops  & 80 - 100 & 53.9 & 80.1 & 59.3\\
%      MoCo-V2 using object and context crops  & 100 - 120 & 53.6 & 80.0 & 59.2\\
%      MoCo-V2 using object and context crops  & 120 - 140 & 53.6 & 80.1 & 60.0\\
%      MoCo-V2 using object and context crops  & 140 - 160 & 53.7 & 80.1 & 59.6\\ 
%         \bottomrule
%     \end{tabu}
%     \caption{Impact of varying radius and using all three modalities. The models have been pre-trained on COCO dataset and then transferred to VOC.}
%     \label{tab:voc_analysis_radius}
% \end{table*}













% \begin{figure*}[h!]
%   \centering
%   \begin{subfigure}{\linewidth}
%     \includegraphics[width=\linewidth]{LaTeX/Images/bing.pdf}
%   \end{subfigure}
%   \caption{This figure shows original image, the object extracted from BING model and the context image. }
%   \label{fig:bing_crops}
% \end{figure*}

% \begin{figure}[h!]
%   \centering
%   \begin{subfigure}{\linewidth}
%     \includegraphics[width=\linewidth]{LaTeX/Images/openimages_crop.pdf}
%   \end{subfigure}
%   \caption{This figure shows original image, and the two random crops. We can see that these random crops often miss the main object and may capture non-relevant background information. }
%   \label{fig:random_crops}
% \end{figure}

